Rapidly-Exploring Quotient-Space Trees: Motion Planning using Sequential Simplifications

Motion planning problems can be simplified by admissible projections of the configuration space to sequences of lower-dimensional quotient-spaces, called sequential simplifications. To exploit sequential simplifications, we present the Quotient-space Rapidly-exploring Random Trees (QRRT) algorithm. QRRT takes as input a start and a goal configuration, and a sequence of quotient-spaces. The algorithm grows trees on the quotient-spaces both sequentially and simultaneously to guarantee a dense coverage. QRRT is shown to be (1) probabilistically complete, and (2) can reduce the runtime by at least one order of magnitude. However, we show in experiments that the runtime varies substantially between different quotient-space sequences. To find out why, we perform an additional experiment, showing that the more narrow an environment, the more a quotient-space sequence can reduce runtime.

==> comments.tex <==
[x] redo picture 1, make them all x instead of q

[ ] Publish @ArXiV and @Medium, call it Hierarchical Motion Planning, Write Blog Post

[ ] Publish OMPL code (after published on ArXiV/Hal)

[x] this is a set, not a tuple

-- Changed: disjoint union

[x] don't use $|\ $ as condition bar, use $\mid$ or $~|~$

%(1) You did not really address the comments given at the lab meeting. You still use subspaces, and confuse them with quotient-spaces.

%(2) QRRT is simpler to understand as a contribution, make this your major
%contributor

%(3) Experimental section was unclear. What did i wanted to do? It felt that
%insight came at the end

%(4) You need to showcase it more consistently, i.e. there should be a clear
%demarcation between technical and evaluation part.

%(5) CR is too basic and should be removed

%(6) In a subspace, every element is still high-dimensional (just constrained). 

%(7) Constraint function is problematic. If it is the feasibility function, then
%its outcome should be $latex 1$ if it is feasible. I.e. otherwise we need to name it
%non-feasibility function. Consider naming it constraint function, then we can
%define it whatever we like.

%(8) Quotient space, not subspace

(9) It is unclear which coordinates we will use for QS

%(10) A projection is $latex \pi$, not a tuple. Consider naming the tuple
%simplification. 

%(11) The canonical simplification will play a major rule, but i dont consider it

%(12) Simplifications (S) instead of strats 

%(13) Eq classes of S after definition of QRRT 

%(14) For simplifications, new A which we call QRRT

%(15) Eq. classes into empirical part

%(16) Tree T instead of graph G. If a priority queue, then what number would we
%add. Unclear!

%(17) Comments in Algorithm are missing: Line 4: Priority in Qk, Line 6: Least
%sampled S. Line 10: Solution to k, move to k+1
%NOTE: added it to text!

%(18) Experimental part should contain two parts, one where we evaluate naively
%QRRT, and then second where we investigate why some strats work better than
%others

%(19) Consider calling strats Sequential Simplifications

%(20) Part2: Here were some results with simplifications. Now we like to
%understand which one is good choice.

%(21) Maybe at the beginning use trivial vs all (and ignore rest)

%(22) Eq. classes are too obfuscated. I am constructing a specific set of S,
%namely the ones which are computationally efficient. Other S are possible, but
%they would not be efficient because the whole orbit/fibre needs to be sampled.

%(23) Other S are not useful, because they have more complexity in evaluating
%their admissibility.

%(24) Prime reader by saying that canonical S is not a good choice, because their
%admissibility is hard to compute. However, in the context of MP, we can actually
%use the fact that we have kinematic trees to evaluate equivalence classes using
%one single collision query.

%(25) QRRT with efficiently computable S, our results differ a lot over
%experiments. Why? That is part 2.


==> review.tex <==
[x] For theorems, it would be useful to state the exact
theorem. For instance, theorem 2 stated "h is admissible".
What is h? What's the criteria for this to happen? 

[x] The extension of [11] to a single-query planner is
interesting and important. Yet, it is well known that
solutions produced by RRT (as well as PRM) can be/are
sub-optimal, which led to the development of RRT* (and
PRM*) [A]. Is there a reason not to consider QRRT*? 

[x] - p. 13 bottom: "We like" -> "We would like"

[x]  Define what $Y \simeq X_1 $ means in this context


[x] The authors consider multiple types of robots which was
very encouraging. However, for each robot they only
consider one environment and compare to a Vanilla RRT
instead of more advanced versions o the algorithm. I really
appreciated the fact that the authors include examples
where their algorithm does *not* outperform the state of
the art to understand the limits of their work. The
additional experiment regarding the narrow passage is
helpful but may be somewhat misleading - here the narrow
passage is defined in the workspace and not in the c-space.
See [3] for a discussion on different *types* of narrow
passages.

[x] It was not clear to me if all algorithms found a
solution to all cases or if some timed out. If the latter
is true then a success rate should be provided.

[x] Here are several related work that are not mentioned and,
in my mind, are closely related. These may be mentioned in
the text, in related work or in future work as possible
methods to extend this work.

[x] The idea of using multiple subspaces to guide the
search is similar in nature to using multiple heuristics in
search-based planning. See for example [1]. In particular,
the approach suggested is similar to the setting where the
different heuristics do *not* share their progress. I urge
the authors to consider how progress made by one RRT in a
projected space can be used to guide a different RRT in a
different projected space (similar to shared MHA* [1]).

[x]  Sentence before equation 3.1. Using \bigcup

[X] Emphasize fiber first time it is used

[x] Page 7 "The priority will get less" -> "... will be
decreased"

[x] Pages are missing from a lot of references (e.g.,
11,12,16,17,20) 

[x] Overall, the biggest concern about this section is the lack
of comparisons to other algorithms and a lack of any
experiments relating to path quality.

[x] 
The algorithm is creating K seperate trees, comments on the
additional memory usage compared to RRT should be included.

[x] I would suggest to use a running example (similar to
Fig 1) used for all the definitions in Sec. 3.3.

[x] Fig 11 should include error bars
[x] 4.  QRRT
There is neither an explanation for how C_k is calculated
or sampled from, nor how samples from C_k and T_k-1 are
concatenated in GrowQRRT.

[x] The formal exposition should be refined. \pi is a
many-to-one mapping from X to Y. This means that \py^-1 is
a  one-to-many mapping.  In addition, \phi is a one-to-one
mapping from X to {0,1}. Thus for the term
$\phi(\pi^-1(y))$ to be defined, \phi needs to  extends
to take subsets of X as well. This notation problems
cascades throughout the formal exposition and has to be
addressed. Another example where the formalism was sloppy
is after Eq 5.9: 2^J should be 2^|J|.

[x] rewrite 3.6 and beginning of 4

[x] (*) The idea of looking at a projection is similar to MMS
[2,3] with the key difference that here the authors sample
one configuration in the projected subspace while in MMS
the authors use *complete* subspaces as samples.

[x] (*) In the discussion regarding probabilistic completeness,
mention recent work by Kleinbort and Solovey [4] which
revisits the classical RRT proof which was shown to be
incomplete in certain settings [5] 

[1] Sandip Aine, Siddharth Swaminathan, Venkatraman
Narayanan, Victor Hwang, Maxim Likhachev:
Multi-Heuristic A. I. J. Robotics Res. 35(1-3): 224-243
(2016)
[2] Oren Salzman, Michael Hemmer, Barak Raveh, Dan
Halperin:
Motion Planning via Manifold Samples. Algorithmica 67(4):
547-565 (2013)
[3] Oren Salzman, Michael Hemmer, Dan Halperin:
On the Power of Manifold Samples in Exploring Configuration
Spaces and the Dimensionality of Narrow Passages. IEEE
Trans. Automation Science and Engineering 12(2): 529-538
(2015)
[4] Michal Kleinbort, Kiril Solovey, Zakary Littlefield,
Kostas E. Bekris, Dan Halperin:
Probabilistic completeness of RRT for geometric and
kinodynamic planning with forward propagation. CoRR
abs/1809.07051 (2018)
[5] Tobias Kunz, Mike Stilman:
Kinodynamic RRTs with Fixed Time Step and Best-Input
Extension Are Not Probabilistically Complete. WAFR 2014:
233-244

[x] Use hyphens when needed. 
E.g.,	motion planning problems ->   motion-planning
problems
		configuration space paths ->
configuration-space paths 
		
[x]  Define terms first time they are introduces
E.g.,	admissible lower-dimensional simplification
		probabilistically complete

[x] The PTC conditions and connect(x_near, x_rand, T) function
are not given in the experiments.
		
[ ] 1. Intro
Authors refer to previous work dealing with quotient space
planning (11) but give a fairly cursory explanation of
quotient spaces and their use in robot motion planning. A
brief explanation of planning space decomposition and
possibly an example (see 11) would help frame the next
section and the rest of the paper and improve
comprehension.

[x] In figures 3, 5, and 7 the histogram plot is slightly
unclear in what data it shows. Comprehension would be
helped by more explicit captions for all three figures. 

[x] The
text on the graphs in figure 7 is also too small to read.

[x] The “Fixed-Base Spatial” paragraph does not properly
explain the relative performance of RRT (QRRT Trivial) to
QRRT and neither the paragraph, nor the figure caption
properly explain the plots, especially the distinction
between left and middle plots.

